Blockchain Governance: An Empirical Analysis of User Engagement on DAOs

In this note, we examine voting on four major blockchain DAOs: Aave, Compound, Lido and Uniswap. Using data directly collected from the Ethereum blockchain, we examine voter activity. We find that in most votes, the "minimal quorum," i.e., the smallest number of active voters who could swing the vote is quite small. To understand who is actually driving these DAOs, we use data from the Ethereum Name Service (ENS), Sybil.org, and Compound, to divide voters into different categories.

==> macros.tex <==
\usepackage[T1]{fontenc}
\usepackage[latin9]{inputenc}
\usepackage[letterpaper]{geometry}
\usepackage[dvipsnames]{xcolor}
\geometry{tmargin=1in,bmargin=1in,lmargin=1in,rmargin=1in}
%\usepackage{babel}
\usepackage{latexsym}
\usepackage{amstext}
\usepackage{setspace}
%\usepackage[authoryear]{natbib}
\usepackage{bm}
\setstretch{1.45}
\usepackage[hyperfootnotes=false, colorlinks=true, linkcolor=black, urlcolor=Black, citecolor={Blue}]{hyperref}
\usepackage{soul}
\def\cblue{\color{blue}}
\def\ccblue{\color{blue}}
\def\cred{\color{red}}
\def\cgreen{\color{Green}}
\def\cblack{\color{black}}
\usepackage{xfrac}
\usepackage{enumitem}
%\usepackage{subfigure}
\usepackage{array}
\usepackage{caption}
\captionsetup{font=small,labelfont=small}
\usepackage{xspace}
\RequirePackage{snapshot}

\usepackage[multiple]{footmisc} %multiple footnotes


%\usepackage[margin=1in]{geometry}
\usepackage{booktabs}
\usepackage{amsmath,amssymb,amsthm}
\usepackage{nicefrac}
\usepackage{float}
\usepackage{framed}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{stmaryrd}
%\usepackage{pgfplots}

%Colors for the events we consider
\xdefinecolor{eblue}{rgb}{.3,.3,.74}
\xdefinecolor{egreen}{rgb}{.3,.74,.3}
\xdefinecolor{ered}{rgb}{.75,.3,.3}

\newcommand{\cG}{\ensuremath{\mathcal{G}}}
\newcommand{\cA}{\ensuremath{\mathcal{A}}}
\newcommand{\cC}{\ensuremath{\mathcal{C}}}


\newcommand{\grph}[1]{\ensuremath{\cG\inparen{#1}}}
\newcommand{\zo}{\ensuremath{\inset{0,1}}}
\newcommand{\mm}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\vv}[1]{\ensuremath{\vec{#1}}}
\newcommand{\vvu}[2]{\ensuremath{\vec{#1}^{#2}}}
\newcommand{\vvs}[2]{\ensuremath{\vvu{#1}{#2}_i}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\half}{\ensuremath{\frac{1}{2}}}
\newcommand{\defined}{\ensuremath{\stackrel{\textrm{def}}{=}}}
\newcommand{\ie}{\emph{i.e.},~}
\newcommand{\eps}{\ensuremath{\epsilon}}
\newcommand{\inparen}[1]{\ensuremath{\left( #1 \right)}}
\newcommand{\inbrak}[1]{\ensuremath{\left[ #1 \right]}}
\newcommand{\inset}[1]{\ensuremath{\left\{ #1 \right\}}}
\newcommand{\MV}{\ensuremath{\mathsf{market}}}
\newcommand{\F}{\ensuremath{\mathsf{failures}}}
\newcommand{\SF}{\ensuremath{\mathsf{shortfall}}}
\newcommand{\BC}{\ensuremath{\mathsf{bailout}}}
\newcommand{\suchthat}{\ensuremath{~\middle|~}}
\newcommand{\updt}{\ensuremath{\mathsf{updated}}}
\newcommand{\shortfall}{\ensuremath{\mathsf{shortfall}}}
\newcommand{\numFailed}{\ensuremath{\mathsf{numFailed}}}
\newcommand{\hp}{\ensuremath{*}}
\newcommand{\smin}{\ensuremath{s_{\mathrm{min}}}}
\newcommand{\share}[1]{\ensuremath{\left\llbracket #1 \right\rrbracket}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\ZZ}[1]{\ensuremath{\Z/#1\Z}}
\newcommand{\Adj}{\ensuremath{\operatorname{Adj}}}
\newcommand{\argmax}{\ensuremath{\operatorname{argmax}}}
\newcommand{\wt}{\ensuremath{\operatorname{wt}}}
\newcommand{\lambdamax}{\ensuremath{\lambda_{\mathrm{max}}}}
\newcommand{\view}[1]{\ensuremath{\mathsf{view}_{#1}}}
\newcommand{\given}{\ensuremath{~\middle|~}}
\newcommand{\imax}{\ensuremath{i_{\mathrm{max}}}}
\newcommand{\bigoh}{\ensuremath{\mathcal{O}}}
\newcommand{\pup}[2]{\ensuremath{#1^{\inparen{#2}}}}
\newcommand{\Da}{\ensuremath{\Delta_A}}
\newcommand{\Db}{\ensuremath{\Delta_B}}
\newcommand{\pl}{\ensuremath{p_\ell}}
\newcommand{\pu}{\ensuremath{p_u}}


\usepackage{tikz}
\usetikzlibrary{calc}

%\theoremstyle{definition}
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{definition}{Definition}
\newtheorem{observation}{Observation}
\newtheorem{remark}{Remark}

\newcounter{question}
\newenvironment{question}[1][]{\refstepcounter{question}\par\medskip\textbf{Question~\thequestion}. #1}{\medskip}

\newcounter{openquestion}
\newenvironment{openquestion}[1][]{\refstepcounter{openquestion}\par\medskip\textbf{Open Question~\theopenquestion}. #1}{\medskip}


%\usepackage{hyperref}

%\hypersetup{
%	colorlinks=true,
%	linkcolor=black,
%	citecolor=black,
%	urlcolor=black
%}

\newcommand{\marcella}[1]{{\color{blue}#1 --Marcella}}
\newcommand{\brett}[1]{{\color{red}#1 --Brett}}
\newcommand{\david}[1]{{\color{green}#1 --David}}
%\newcommand{\gt}[1]{{\color{magenta}#1 (GT)}}
\newcommand{\gt}[1]{{\color{magenta}#1}}
\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}}

\usepackage{graphicx}
\graphicspath{{./code/mpyc/src/} {figures_}}
\usepackage{subcaption}
\usepackage{cleveref}

%\usepackage{natbib}
% \bibpunct[, ]{(}{)}{,}{a}{}{,}%
% \def\bibfont{\small}%
% \def\bibsep{\smallskipamount}%
% \def\bibhang{24pt}%
% \def\newblock{\ }%
% \def\BIBand{and}%
% \def\red{\color{red}}
%\def\cblack{\color{black}}


